Data-Centric and Data-Aware Frameworks for Fundamentally Efficient Data Handling in Modern Computing Systems

There is an explosive growth in the size of the input and/or intermediate data used and generated by modern and emerging applications. Unfortunately, modern computing systems are not capable of handling large amounts of data efficiently. Major concepts and components (e.g., the virtual memory system) and predominant execution models (e.g., the processor-centric execution model) used in almost all computing systems are designed without having modern applications' overwhelming data demand in mind. As a result, accessing, moving, and processing large amounts of data faces important challenges in today's systems, making data a first-class concern and a prime performance and energy bottleneck in such systems. This thesis studies the root cause of inefficiency in modern computing systems when handling modern applications' data demand, and aims to fundamentally address such inefficiencies, with a focus on two directions. First, we design SIMDRAM, an end-to-end processing-using-DRAM framework that aids the widespread adoption of processing-using-DRAM, a data-centric computation paradigm that improves the overall performance and efficiency of the system when computing large amounts of data by minimizing the cost of data movement and enabling computation where the data resides. Second, we introduce the Virtual Block Interface (VBI), a novel virtual memory framework that 1) eliminates the inefficiencies of the conventional virtual memory frameworks when handling the high memory demand in modern applications, and 2) is built from the ground up to understand, convey, and exploit data properties, to create opportunities for performance and efficiency improvements.

==> 0_abstract.tex <==

%%%% VIVEK

% Memory systems continue to diversify with respect to application demands and emerging memory technologies. Continually adapting the conventional virtual memory framework for each possible use case is challenging and often results in performance loss or requires non-trivial complex workarounds. 

% \onurthird{To address this problem, we propose an alternative virtual memory framework called the \sysfull (\sys). \sys is driven by three key design principles: (1)~applications should be allowed to choose the size of their virtual address space, (2)~address translation should be decoupled from memory protection, and (3)~the virtual memory framework should communicate semantic information about the application data to the hardware. Based on these principles, our first idea is to design a data-structure-centric virtual memory interface that allows applications to allocate each of their data structures in a separate \emph{virtual block}. To this end, \sys exposes a global set of virtual blocks of various sizes to software. Our second idea is to use a hardware-based \mtlfull (\mtl) to perform both physical memory allocation and address translation. The OS only controls which programs have access to which virtual blocks.}

% We demonstrate the benefits of \sys using  two important use-cases: (1)~a virtual machine environment and (2)~two heterogeneous memory architectures.  We show that VBI naturally suits both scenarios, and significantly improves performance relative to a conventional virtual memory framework.


%%%% ALTERNATIVE

Computers continue to diversify with respect to system designs, emerging memory technologies, and application memory demands. Unfortunately, continually adapting the conventional virtual memory framework to each possible system configuration is challenging, and often results in performance loss or requires non-trivial workarounds. 

% \sys uses hardware-based memory allocation and address translation to create a highly flexible framework.
% \sys introduces a global set of variable-sized virtual blocks (VBs), which are allocated and mapped to physical memory by hardware. \sys decouples memory allocation from memory protection (which is still handled by the OS), and uses system-wide unique addresses for VBs that avoid using address translation to disambiguate between virtual addresses.  This allows \sys to enable several architectural optimizations that cater better to the needs of each application, and eliminate many of the inefficiencies of conventional memory allocation and address translation.}


% \sys manages virtual memory in variable-sized regions known as virtual blocks (VBs) that are mapped to processes by the system software and 
%\sys treats all allocated virtual memory as part of a global set of variable-sized virtual blocks (VBs) that the OS can attach to processes based on needs and access permissions (e.g., private, shared). Unlike conventional systems, \sys delegates the physical memory management duties (including memory allocation and virtual-to-physical address translation) to dedicated hardware within the memory controller. Because VBs are unique system-wide, \sys enables several architectural optimizations that can efficiently and flexibly cater to the particular needs of each application and eliminate key inefficiencies of conventional virtual memory frameworks.

%% Nastaran
% a few notes
% - avoid the word firmware, we are not using it anymore
% - vbi decouples "address translation" and "memory protection"
% - MTL does not do virtual-to-physical address translation, it does VBI-to-physical address translation
% - VBI addresses and VBI address space are not exposed to the applications. only VBs are (with an indirection).

To address these challenges, we propose a new virtual memory framework, the \sysfull (\sys). We design \sys based on the key idea that delegating memory management duties to hardware can reduce the overheads \onurii{and software complexity} associated with virtual memory. \sys introduces a set of variable-sized virtual blocks (VBs) to applications. Each VB is a contiguous region of the globally-visible \emph{VBI address space}, and an application can allocate each %data structure
\onurv{semantically meaningful unit of information (e.g., a data structure)} in a separate VB. 
% \sys decouples memory management from access protection:
% we add hardware in the memory controller to manage physical memory allocation and address translation for VBs, while we use the OS to control which programs have access to which VBs. 
% % While the OS manages which programs have access to which VBs, \sys manages the physical memory allocation and address translation of the VBs using dedicated hardware. 
% % The hardware based memory management together with OS-managed access protection 
% Our mechanism provides several architectural optimizations to (1)~efficiently and flexibly cater to the particular needs of different system configurations, and (2)~eliminate key inefficiencies of conventional virtual memory frameworks.}
\sys decouples access protection from memory allocation and address translation. While the OS controls which programs have access to which VBs, \onurii{dedicated hardware in the memory controller} manages the physical memory allocation and address translation of the VBs. This approach enables several architectural optimizations to (1)~efficiently and flexibly cater to \onurii{different and increasingly diverse system configurations}, and (2)~eliminate key inefficiencies of conventional virtual \onurv{memory}.


% \onurthird{To address this problem, we propose an alternative virtual memory framework called the \sysfull (\sys). We design \sys based on two key principles: (1)~data-structure-oriented virtual memory management, which enables significant flexibility to adapt to different system configurations and application demands; and (2)~hardware-based address translation and memory allocation, which 
% % decouples address translation from memory protection and
% % together with OS-managed access protection 
% reduces the overheads associated with virtual memory.
% % To this end, 
% \sys introduces a global set of variable-sized virtual blocks (VBs), where the VBs employ system-wide unique memory addresses.
% % are uniquely addressed within the memory hierarchy.
% % form a the globally-visible \emph{VBI address space} which consists of a set of variables sized \emph{Virtual Blocks (VBs)}. 
% With VBs, an application can efficiently allocate each of its data structures in a separate VB.
% % \sys allows an application to efficiently allocate each of its data structures in a separate VB, and 
% \sys manages the main memory allocation and address translation of the VBs using 
% % a hardware \mtlfull (\mtl) that resides within the memory controller. 
% hardware and firmware in the memory controller, which enables several optimizations for virtual memory management.
% In \sys, the OS retains full control over access protection by managing which programs have access to which VBs.}

We demonstrate the benefits of \sys \onurii{with} two important use cases: (1)~reducing the overheads of address translation (for both native execution and virtual machine environments), as \sys reduces the number of translation requests and associated memory accesses; and (2)~two heterogeneous \onurii{main} memory architectures, where \sys increases the \onurii{effectiveness} of managing fast memory regions.  For both cases, VBI 
% naturally suits both scenarios, and 
significantly improves performance \onurii{over} conventional virtual memory.


==> 2_old_design_principles.tex <==
\section{Design Principles}
\label{sec:design-principles}

VBI is grounded on three key design principles: 


\noindent
\textbf{Size of the Virtual Address Space.} The majority of applications far underutilize the large virtual address space offered by modern architectures (e.g., 256~TB in Intel \xeightsix). Even high-performance applications such as databases~\cite{db1,db2,db3,db4,db5,db6} and caching servers~\cite{memcache,memcached1} are cognizant of the amount of available physical memory and of the size of virtual memory they need. Unfortunately, a larger virtual address space leads to a larger address translation overhead as it results in deeper page tables, so each TLB miss requires more page table accesses to retrieve the physical address. %and (2) increased contention at address translation hardware structures (e.g., TLBs). 
Therefore, we need a framework that allows programs to choose an appropriately-sized virtual memory address space.
 

\noindent
\textbf{Address Translation vs. Access Protection.} Address translation and access protection checks have different characteristics. While address translation is typically performed at page granularity, protection information is typically the same for an entire data structure that can span many pages. Moreover, protection information is purely a function of the virtual address and does not require address translation. Unfortunately, existing systems couple address translation and data protection. Decoupling the two can remove address translation from the critical path of an access protection check, enabling opportunities to reduce translation overhead (e.g., using fully virtual caches).

\noindent
\textbf{Software vs. Hardware.}  Data structures vary greatly in size, have different performance characteristics (latency, bandwidth, and parallelism), and have other inherent properties (compressibility, persistence, etc.) at the software level. As highlighted by recent work~\cite{xmem}, while software is aware of this semantic information, the hardware is privy to dynamic runtime information (i.e., memory behavior, phase changes, bandwidth availability, etc.) that can enable vastly more intelligent management of the underlying hardware resources (i.e., better data mapping, migration, and scheduling decisions). Therefore, a framework that enables software to easily communicate semantic information to hardware and allows hardware to manage the memory mapping and allocation can enable a host of new optimization opportunities.



==> 3_old_vbi_high_level.tex <==
\section{The Virtual Block Interface}
\label{sec:overview}

The goal in \sys, as an alternative virtual memory framework, is to enable a flexible platform for efficient adoption of the diverse recent system designs, emerging memory technologies, and modern applications while addressing the shortcomings of the conventional virtual memory framework. In this section we describe in high-level how \sys achieves this goal using the above design principles.


\subsection{\sys: High Level Design and Semantics}
\label{sec:high-level-design}

\sys hides the details of the underlying physical memory and exposes a \emph{globally-visible} address space called \emph{VBI address space} to the rest of the system, including the OS. The VBI address space consists of a \emph{global} set of Virtual Blocks (VBs). A VB is a contiguous region of VBI address space that \emph{does not overlap} with any other VB. The global set of non-overlapping VBs makes each VB unique system-wide and leads to the system-wide-visible VBI address space. in \sys, each VB is identified globally using a unique ID. The combination of the unique ID of the VB and the offset within the VB creates a unique address in the VBI address space, which we call the \emph{VBI address}. \sys supports VBs of multiple different sizes ranging from 4~KB to 128~TB, and each VB is associated with a set of \emph{properties} that describe the semantics of the VB's contents~(\secref{sec:vb-detail}). Our idea behind this approach is that each process (including the OS) may map each unit of semantically meaningful information (e.g., data structures, libraries) to a \emph{separate} virtual block of an appropriate size. 
In \sys, each VB can attach to any number of VBs. Accordingly, the address space of a process consists of the set of VBs that it is attached to. Figure~\ref{fig:design-overview} gives an example of a data-structure-to-VB mapping for two programs (one running natively and another running inside a virtual machine).

This approach allows 1)~each process to maintain an appropriately sized virtual address space that the application \emph{actually requires} (first design principle), 2)~the OS to manage memory protection and sharing semantics at the granularity of VBs, and the \mtl to manage the address translation by maintaining a separate translation structure for each VB and tune it to the needs of the VB (second design principle), and 3)~~a process to easily communicate semantic information about each of its data structures to the hardware using the VB properties (e.g., VB3 and VB6 in Figure~\ref{fig:design-overview} are marked as latency-sensitive (\emph{l/s}) and bandwidth-sensitive (\emph{b/s}) respectively) (third design principle).



\subsubsection{Access Semantics}
\label{sec:access-semantics}

To enable a program to access its data, protect its data from other programs, or share data efficiently with other programs, \sys imposes the following access semantics: a program can access a VB \emph{only if} it is attached to the VB with appropriate permissions. %For example, 
In Figure~\ref{fig:design-overview}, \textsf{Program 2} can only execute from \textsf{VB 4} or \textsf{VB 5}, only read from \textsf{VB 6}, and cannot access \textsf{VB 3} at all; \textsf{Program 1} and \textsf{Program 2} both share \textsf{VB 4}. \sys gives the OS full control over mapping permissions from programs to VBs.


\begin{figure}
    \centering
    \scalebox{0.8}{\input{figures/vbi-overview-new.tex}}
    \caption{Overview of \sys Design. (l/s) and (b/s) represent latency-sensitive and bandwidth-sensitive
respectively.}
    \label{fig:design-overview}
    \vspace{-10pt}
\end{figure}

\subsubsection{Virtual Block to Physical Memory Translation}
\label{sec:vb-pm}


Since the VBI address is unique system-wide, it can be directly used to address caches, thereby eliminating the need to perform address translation for all on-chip cache accesses. This enables \sys to delay the address translation to when the physical memory needs to be accessed. Accordingly, 
\sys shifts VBI-to-physical address translation duties to the \mtlfull (\mtl) in the memory controller, right before %as the point where the 
an access to main memory.

\sys replaces the rigid structure of page tables with a \emph{separate} address translation structure for \emph{each VB} that can be tuned to suit the characteristics of the VB (e.g., multi-level tables for large or sparsely-populated VBs and single-level tables or direct map for small or densely-populated VBs)~(\secref{sec:flexible-translations}).

\subsection{Implementing Key OS Functionalities}
\label{sec:os-functions}

%\subsubsection{Physical Memory Capacity Management}
\textbf{Physical Memory Capacity Management.} As described in the previous section, the MTL completely manages physical memory in \sys. It allocates physical memory for newly-active VBs as and when required, and it frees physical memory when an active VB is disabled. With the advent of large non-volatile memory technologies, we envision that many systems will no longer need separate \emph{swap files}~\cite{linux-swap}, making such MTL-based management possible
without any interaction with the OS. 
However, it is straightforward to enable a system call to allow the MTL to move data to the backing store with the help of the OS. The \mtl exposes the least-recently-used VBs to the OS, which uses this information to swap parts of VBs out of the main memory to a backing store. The \mtl maintains information on the swapped-out regions as part of the VB's translation structures. On a subsequent access to a swapped-out region, the \mtl interrupts the OS to bring the region back to main memory.

%\subsubsection{Data Protection}
\textbf{Data Protection.} The goal of data protection is to prevent a malicious program from accessing kernel data or the private data of other programs. In \sys, every memory allocation (e.g., code, data) is encapsulated in a VB, and a program is not able to generate the addresses within a VB that it is not attached to. Furthermore, the OS ensures protection guarantees by appropriately setting the permissions with which each process can access different VBs. Before each instruction or memory access, the CPU checks if the executing thread has appropriate access permission to the corresponding VB (Section~\ref{sec:load}).


%\subsubsection{Inter-process Data Sharing (True Sharing)}
%\label{sec:true}
\textbf{Inter-process Data Sharing (True Sharing). }
When two processes share data (e.g., via pipes), both processes have a coherent view of the shared memory; i.e., modifications made by one process should be visible to another process. In \sys, the OS supports such \emph{true} sharing by granting both processes permission to access the VB containing the shared data. %For instance, 
In Figure~\ref{fig:design-overview}, VB 4 is shared between both processes 1 and 2.

%This approach to true data sharing eliminates the need for \emph{synonyms} (i.e., two \emph{different} virtual addresses mapped to the \emph{same} physical address) as both processes use the same virtual address to access the shared physical memory.

%\subsubsection{Data Deduplication (Copy-on-Write Sharing)}
\textbf{Data Deduplication (Copy-on-Write Sharing). }
In most modern systems, the OS reduces redundancy in physical memory by mapping multiple virtual pages that contain the \emph{same} data to the same physical page and by periodically coalescing duplicate pages throughout the physical memory.
On a write access to a deduplicated virtual page, the OS copies the contents of the physical page to a new physical page and remaps the written virtual page to the new physical page in order to apply the changes. In \sys, the MTL manages such copy-on-write sharing using a similar mechanism to the existing systems. The OS simply informs the \mtl of events when a virtual block is cloned. In response, the \mtl appropriately copies the mapping information from the original VB to the copy VB and shares the physical pages between the two VBs, following the copy-on-write principle to avoid aliasing. 

%\subsubsection{Memory-mapped Files}
\textbf{Memory-mapped Files. }
Most modern systems support memory-mapped files, wherein a region of the virtual address space is mapped to a file in storage. This allows the system to seamlessly convert loads/stores to that region of the address space into file reads/writes. \sys naturally supports such memory-mapped files as the OS simply associates the file to a VB of appropriate size. An offset within the VB maps to the same offset within the file.

\subsection{ Optimizations Supported by \sys}
\label{sec:optimizations}

\textbf{Avoiding 2D Page Walks in Virtual Machines. }
Section~\ref{sec:virtual-machines} discuss the implementation of this optimization. In \sys, after a VM attaches to its VBs, any access made by the VM to those VBs accesses all on-chip caches using the globally-unique VBI addresses, without requiring the guest or host OS to perform address translation. Accesses that miss in all levels of the cache and reach the physical memory are then translated to physical addresses only once by the MTL located at the memory controller. As a result even accesses generated by a VM go through only one round of address translation at the MTL. This yields greater savings in environments that make use of nested virtualization~\cite{google-nested,azure-nested}. Section~\ref{sec:virtual-machines} discusses how we implement this optimization.

\textbf{Virtually-Indexed Virtually-Tagged (VIVT) Caches.} Using VIVT caches in the CPU can enable the system to delay address translation and alleviate high-pressure translation devices such as the TLB. However, most modern architectures do not support VIVT caches due to 1)~the complexity of handling homonyms and synonyms~\cite{cekleov1997a, cekleov1997b, jacob1998}, and 2)~the necessity of a page walk before accessing the cache in case of TLB miss to perform permission check even though address translation is not required, since protection bits are stored as part of the page table entry for each page in current systems. VBI avoids both of these problems.

First, VBI addresses are unique system-wide, eliminating the possibility of homonyms. Furthermore, since VBs do not overlap, each VBI address appears in \emph{at most one} VB, hence, eliminating synonyms. In case of true sharing, different processes are attached to the same VB. Therefore, the VBI address that each process uses to access the shared region refers to the same VB, which eliminates synonyms~(\secref{sec:os-functions}). In case of copy-on-write sharing, where the MTL may map two VBI addresses to the same physical memory for deduplication, the MTL creates a new copy of the data before any write to either address, thereby eliminating the possibility of synonyms.
As a result, VBI addresses can be directly used to access on-chip caches without the complexity of dealing with synonyms and homonyms. Additionally, since the VBI address acts as a system-wide single point of reference for the data that it refers to, all coherence-related requests can be issued using only the VBI addresses without introducing any ambiguity.

Second, \sys decouples protection checks from address translation, by storing protection and address translation information in \emph{separate} sets of tables and delegating access permission management to the OS.

%Our implementation overlaps address translation with last-level cache access, effectively hiding the address translation latency, while still significantly reducing the number of address translation requests.



\textbf{Delayed Physical Memory Allocation.} As \sys uses VBI addresses to access all on-chip caches without requiring translation to physical addresses, it is no longer necessary for a cache line to be backed by physical memory \emph{before} it can be accessed. This enables the opportunity to delay physical memory allocation for a VB (or a region of a VB) until a dirty cache line from the VB is evicted from the on-chip last-level cache. Delayed allocation has three benefits. First, the allocation process is removed from the critical path of execution, as cache line evictions are not on the critical path. Second, for VBs that never leave the cache during the lifetime of the VB (common with the growing cache sizes in modern hardware), \sys avoids physical memory allocation altogether. Third, for an access to a region with no physical memory allocated yet, \sys simply returns a zero cache line, thereby avoiding both address translation and a main memory access, which in turn improves performance.

\textbf{Flexible Translation Structures.} As shown by recent work~\cite{vm19}, different data structures benefit from different types of translation structures depending on their data layout and access patterns. %For instance, while multi-level page tables are a good choice for a sparsely allocated data structure, they consume unnecessary space and page walks for a densely allocated VB. 
However, since in most virtual memory frameworks hardware needs to read the OS managed page tables in order to perform page table walks, the structure of the page table is a rigid and inflexible contract between OS and the hardware. In contrast, the \mtl is the \emph{only} component in \sys that manages and accesses translation structures. Therefore, by maintaining a \emph{separate} translation structure for each VB, \sys tunes the type of translation structure to suit the properties of the VB (e.g., multi-level tables for large or sparsely-populated VBs and single-level tables for small or densely-populated VBs). This optimization reduces the number of memory accesses necessary to serve a TLB miss.


% \subsection{\sys vs Prior Work}
% \label{sec:key_idea}


% \textbf{Key Idea. }The key idea of VBI is to use hardware-based physical memory allocation and virtual-to-physical address translation, which to the best of our knowledge, has not been explored by prior work. The MTL in VBI manages physical memory allocation and address translation for all OSes (guests or host) in the system, differentiating VBI form prior works that require operating system support for these operations (e.g., single address space OSes, segments, enabling VIVT caches). VBI’s approach enables three major benefits that are not straightforward in prior works: (1) single-level address translations in virtualized systems, since address translation is transparent with respect to guest and host OS; (2) delayed physical memory allocation, since acquiring the physical address is required only at the MTL (i.e., at the memory controller) and only to access the physical memory%Implementing such a technique in current systems with VIVT caches needs costly OS interventions on every cache eviction to allocate a page
% ; and (3) providing applications with the familiar view of a private address space while exposing hardware, but not processes, to a unified address space, thereby enabling key performance optimizations (e.g., VIVT caches, address translation off the critical path of cache access).


% \textbf{\sys vs Segmentation. }While VBs may resemble segments from an application’s perspective (i.e., an additional indirection between application addresses and the VB address space), VBI does not require the OS to manage physical memory resources. Unlike in segment-based architectures, VBI puts the physical memory entirely in the purview of the hardware-based MTL, which the OS interacts with in order to coordinate the VB address space rather than directly managing it. Furthermore, VBs convey semantic information about the data they contain, which enables more intelligent memory allocation and usage.





==> 4_old_vbi_detailed_description.tex <==
\section{\sys: Detailed Design}
\label{sec:detailed}


\subsection{Architectural Interface}
\label{sec:arch-interface}

VBI offers \emph{memory clients} (i.e., user processes, operating system) a virtualized memory interface through globally unique \emph{virtual blocks}. This section describes how virtual blocks are implemented and how memory clients make use of them.

\subsubsection{Virtual Blocks}
\label{sec:vb-detail}

\sys is characterized by three parameters: 1)~\shepherd{the total size of the VBI address space, which is determined by the number of bits of virtual address used by the processor (64 in our implementation)}, 2)~the number of virtual block size classes (8 in our implementation), and 3)~the list of size classes---4~KB, 128~KB, 4~MB, 128~MB, 4~GB, 128~GB, 4~TB, and 128~TB.\footnote{This is an example set and number of size classes that we use in our evaluations while VBI can be designed around any set of size classes} Each VB in \sys has a unique ID within its size class. The ID of the VB together with the ID of the size class that it belongs to \emph{uniquely} identify the VB throughout the system. \shepherd{\sys constructs a \emph{globally unique} 64-bit \emph{VBI address} using three components: (1) the ID of the size class, (2) the ID of the VB within the size class, and (3) the offset of the addressed block within the VB.}

In \sys, each virtual block is associated with a \emph{separate} translation structure, a set of properties inherent to its contents represented as a bit vector (e.g., code, read-only data, persistent data), and the dynamic status of the VB (e.g., whether the VB is active, the number of processes attached to the VB).  All these pieces of information are stored in a set of \emph{VB Info Tables}~(\secref{sec:vit}). VB properties can theoretically be any hint from the software to the hardware, such as access pattern (e.g., regular/irregular), access intensity (i.e, hotness of data), or data locality (e.g., reuse frequency). Prior work extensively studies useful properties~\cite{xmem}, and we expect system designers to use VBI with any such properties that are useful in the context of a given system. 


\subsubsection{Memory Clients} 
\label{sec:client}

In \sys, \emph{any} entity that needs to allocate and use memory is referred to as a \emph{memory client}. Examples of memory clients include the OS itself and any process that is running natively on the system or inside a virtual machine. In order for the OS to maintain and track the permissions with which each process can access different VBs, 
each client in \sys is assigned a \emph{memory client ID}\footnote{Similar to the unique ASID used in current systems.} to identify the client system-wide. 
During execution, \sys tags each hardware thread with the client ID of the process running on it, enabling the processor to perform access control checks. The set of VBs that can be accessed by a client and their corresponding permissions are stored in a \emph{per-client} table called \emph{Client VB Table} (CVT), managed by the OS. Each CVT entry stores a valid bit for the entry, the ID of a VB, and the permissions with which the client can access that VB. For \emph{each} client, the processor maintains the location and size of the CVT in a reserved region in memory (512~KB for $2^{16}$ clients). As the client ID is hardware-visible, the number of clients is an architectural parameter determined at design time and exposed to the OS. In our implementation, we use 16-bit client IDs (supporting $2^{16}$ clients).

\subsubsection{Address Generation}
\shepherd{While the simplest way for a process to access a VB would be to use a direct addressing mode that specifies the target VB. such an approach results in several issues with marinating the validity of the pointers and compile time addresses in scenarios where the unique ID of the VB changes. For instance, our system allows the process to promote a VB to a higher size class when the VB needs more physical memory space~(\secref{sec:resize}). When the VB is promoted to a new size class, the unique identifier of the new VB (i.e., the combination of the size class ID and VB ID) is different from that of the old VB. If a process uses VBI addresses to directly access VBs, all of the pointers present in the old VB are stale in the new VB, as they are relative to the unique ID of the old VB. The same issue occurs in (1) cloning VBs when forking a new process, where the content of the parent VBs are copied to the child VBs but child VBs do not have the same VB ID; and (2) sharing library code between multiple processes, where library code contains references to the data VB that is private to each process and has a different VB ID.}

\shepherd{In order to address the issue of stale pointers in such cases, a process in \sys \emph{indirectly} specifies the target VB, and the processor maps the process-specified address to the corresponding VB prior to accessing the cache. When a process attaches to a VB, it receives the index of the VB in the process' \cvt (\secref{sec:dynamic_alloc}). In order to access the data inside the VB, the process then generates a virtual address in the format $\{${\tt \cvt index, offset}$\}$, where the \texttt{offset} is the location of the data inside the VB~(\secref{sec:load}). For each memory operation, the processor uses the \texttt{CVT index} in the virtual address to index into the \cvt and retrieve the target VB ID and size class ID. The processor then 1)~performs the access permission check using the \texttt{CVT index}, and 2)~constructs the VBI address, which takes the format $\{${\tt size class ID, VB ID, VB offset}$\}$ (\secref{sec:vb-detail}). The VBI address is used to access all on-chip caches, and is translated to the memory-visible physical address at the \mtl whenever off-chip main memory needs to be accessed. Figure~\ref{fig:virtual-address} shows the lifetime of an address in \sys, with a 10-bit \cvt index.}

\shepherd{As a result of this indirection when addressing the target VB, the compile-time addresses in \sys (i.e., program virtual addresses) are independent of the VB ID. This enables two key properties in \sys. First, \sys does not require relocatable code to maintain the validity of pointers when copying and migrating VBs across the physical memory. The pointers stay valid in any other VB as long as the CVT index of the VB remains the same. %Second, \sys avoids issues associated with single-address-space operating systems which are due to the shared virtual address space among all processes (e.g., shared libraries with per-process private data).  virtual addresses relative to \cvt index that can map to different VBs for each process.  Third, }
Second, \sys provides the processes with a familiar view of a private per-process virtual address space, while addressing the hardware (including all on-chip caches) using a globally-visible VBI address space. The system-wide unique VBI addresses enable key performance optimizations, such as VIVT caches with no synonyms and homonyms, and delaying the address translation until accessing physical memory is required. Section~\secref{sec:pop-interaction} describes how addressing the target VB indirectly helps VBI maintain the validity of the pointers when cloning VBs or sharing library code between multiple processes.}

\begin{figure}[h]
  \centering
  \vspace{-10pt}
   \includegraphics[width=\linewidth]{VBI_ISCA2020/figures/figure3.pdf}
  \caption{\shepherd{Three types of addresses used in VBI.}}
  \label{fig:virtual-address}
  \vspace{-10pt}
\end{figure}

As Figure \ref{fig:virtual-address} shows, \sys supports a greater number of small VBs, whose shorter offset fields leave more bits for the VB ID. Assuming 4KB VBs with 12 bits of offset, the VB ID is 49 bits long. As a result, \sys supports up to $2^{49}$ VBs of size 4KB which represents an address space of size $2^{61}$ bits (256 PB), which we do not expect a typical system to exhaust. In the event that all 4KB VBs are consumed, \sys would use the next-largest size for small allocations, resulting in some amount of internal fragmentation. However even in this case, the early reservation technique (\secref{sec:early-reservation}) combined with a sparse address-translation structure ensures that no unnecessary physical memory is allocated.

\subsection{Microarchitectural Implementation and ISA Support}
\label{sec:ISA}

\begin{figure*}[t]
  \vspace{-20pt} 
  \centering
  \includegraphics[scale=0.51]{VBI_ISCA2020/figures/vbi_v3.pdf}
  \vspace{-20pt}
  \caption{Microarchitectural Implementation of the Virtual Block Interface}
  \label{fig:vbi-uarch}
  \vspace{-20pt}
\end{figure*}

Figure~\ref{fig:vbi-uarch} presents the microarchitectural implementation of \sys and the control flows of a memory allocation and load operation. We describe the implementation of VBI mechanism and ISA support using an example of memory allocation and a load operation. 

\subsubsection{Dynamic Memory Allocation}
\label{sec:dynamic_alloc}

As described in \secref{sec:access-semantics}, a client can read/write/execute a VB only if it is attached to the VB with the respective permissions. In \sys, the OS maintains the mapping between the clients (processes) and the VBs by dynamically (1)~providing clients with VBs of the appropriate sizes as per their request, (2)~attaching clients to their VBs with the right permissions, and (3)~detaching clients from the VBs that they do not need anymore. To this end, \sys adds four new instructions to the instruction set architecture.

\begin{center}\footnotesize
\vspace{-3ex}
\renewcommand{\arraystretch}{1}
\setlength{\aboverulesep}{3pt}
\setlength{\belowrulesep}{3pt}
\setlength\tabcolsep{2pt}
\begin{tabular}{rlp{1.85in}}
  \toprule
  \multirow{2}{*}{\textcolor{blue}{\enablevb}} & \multirow{2}{*}{\tt VBID, props} & ; enables the VB \texttt{VBID} with properties vector \texttt{props}\\
  \midrule
  \textcolor{blue}{\disablevb} & \tt VBID & ; disables the VB \texttt{VBID}\\
  \midrule
  \multirow{3}{*}{\textcolor{blue}{\attachvb}} & \multirow{3}{*}{\tt CID, VBID,
    RWX} & ; attaches client \texttt{CID} to VB \texttt{VBID} with permissions
  \texttt{RWX} (3-bit vector)\\
  \midrule
  \textcolor{blue}{\detachvb} & {\tt CID, VBID} & ; detaches client \texttt{CID} from VB \texttt{VBID}\\
  \bottomrule
\end{tabular}
\vspace{-2ex}
\end{center}

\noindent
As shown in Figure~\ref{fig:vbi-uarch}, for each data structure that requires dynamic memory allocation, the program first requests a VB of an appropriate size from the OS using a new system call, \requestvas (\ding{172}). This call takes the requested VB size and a bit-vector of desired VB properties as arguments. In response to \requestvas, the OS first determines the appropriate VB size class based on the requested size. Then, the OS asks the \mtl to enable a free VB of that size class with the necessary properties using the \enablevb instruction (\ding{173}). For this instruction \texttt{VBID} is the unique ID of the free VB. Enabling a VB informs \sys that the VB is now being used by a client to allocate/access memory. Semantically, by receiving the \enablevb instruction, \mtl adds the newly activated VB to the VIT tables, which store information associated with all active VBs in the system~(\secref{sec:vit}). \mtl then informs the OS of the ID of the new VB. Next, the OS attaches the program's client ID to the VB with the appropriate permissions using the \attachvb instruction (\ding{174}). The \attachvb instruction adds a new entry to the CVT of the client (\texttt{CID}), indicating that the client can now access the VB (\texttt{VBID}) with permissions indicated by \texttt{RWX}. The \attachvb instruction then returns the index of the VB in the client's CVT to the OS. The OS in turn returns this index to the client as a response to the \requestvas system call (i.e., \texttt{index} in the code snippet). \shepherd{This index is later used by the client to generate virtual addresses.}

At this point, the client has access to any location within the VB and can \emph{manage} the memory inside the VB using a library that provides a modified version of \texttt{malloc/free}, which also take the \texttt{index} returned by the \requestvas call as arguments to determine the target VB (\ding{175}). 


The \textcolor{blue}{\detachvb} instruction nullifies the entry corresponding to \texttt{VBID} from the CVT of the client \texttt{CID}. The \textcolor{blue}{\disablevb} instruction informs \sys that the VB is not being used anymore and all state associated with it can be destroyed. \secref{sec:vit} discusses the microarchitectural implementation of these two instructions and the VB Info Tables in more detail.

\subsubsection{Operation of a Memory Load}
\label{sec:load}

As shown in Figure~\ref{fig:vbi-uarch}, \shepherd{to perform a load, the program specifies the virtual address of the memory load operation (\ding{202} in the figure), using 1)~the index of the corresponding VB in the CVT of the client (returned by the \requestvas call), and 2)~the offset within the VB (as determined by the compiler, similar to
existing systems)}. As the first step in executing a load, the CPU checks whether the index is within the range of the CVT of the client and fetches the corresponding CVT entry (\ding{203}). It then checks if 1)~the client has permission to read from the VB, and 2)~the offset in the load instruction is smaller than the size of the VB. If any of these checks fail, the CPU raises an exception. \shepherd{If the access is allowed, the CPU constructs the VBI address~(\ding{204}), as discussed in \secref{sec:vb-detail}}.

\shepherd{The VBI address is used to \emph{directly} access the on-chip caches without requiring translation to a physical address~(\ding{205}).} If the data is present in any of the on-chip caches, then it is returned to the processor, thereby completing the load instruction. When an access misses in the last-level cache, the processor must perform address translation to obtain the physical address of the access (\ding{206}). To this end, the \mtl first fetches the pointer to the VB's translation structure from the entry associated with the VB in the VIT table. Next, the \mtl performs the address translation by traversing the translation structure of the VB~(\secref{sec:mtl}). The VIT cache and the TLBs help to speed up the address translation process.
Once the \mtl obtains the physical address, the memory controller fetches the corresponding cache line from main memory and returns it to the processor. \shepherd{The cache line is then inserted into the on-chip caches using the VBI address for the tag and index, and is returned to the core to complete the load}.

\subsubsection{CVT Cache}
\label{sec:cvt}

As the processor must verify access permissions for every memory operation, the CVT access is always on the critical path. To exploit locality in the CVT, \sys uses a per-processor CVT cache local to the CPU to store recently accessed entries in the client's CVT. The CVT cache is very similar to the TLB in existing processors. However, unlike a TLB that caches virtual-to-physical address mappings of page-sized memory regions, the CVT cache maintains information at the VB granularity and only for VBs that can be accessed by the program. While programs may typically access hundreds or thousands of pages, our evaluations show that most programs only need a few \emph{tens} of VBs to subsume all their data. In our evaluations, with the exception of \texttt{GemsFDTD} which allocates 195 VB\footnote{GemsFDTD performs computations at the time domain on 3D grids. It involves multiple execution timesteps and during each, new 3-D grids are allocated to store the computation output. Multiple allocations are also needed during the post-processing Fourier Transformation performed in GemsFDTD.}, all applications use less than 48 VBs. This means that the processor can achieve a near-100\% hit rate even with a 64-entry \emph{direct-mapped} CVT cache, which is faster and more efficient than the large set-associative TLBs employed by modern processors. Therefore, \sys can perform access protection checks with lower overhead on the critical path of the access when compared with existing systems. Similar to a page lookup during a permission-check-triggered TLB miss in current systems, the CVT lookup is performed only in the case of a miss in the processor's CVT cache, which is stored locally to the CPU. 


\subsection{Processor, OS, and Process Interactions}
\label{sec:pop-interaction}

\sys handles basic process lifetime operations similarly to how current systems do so. This section describes in detail how these operations work with \sys.

\noindent
\textbf{System Booting. }
When the system is booted, the processor initializes the data structures relevant to \sys (e.g., pointers to VIT tables) with the help of the Memory Translation Layer (discussed in \secref{sec:mtl}). An initial ROM program runs as a privileged client and copies the bootloader code from bootable storage to a newly enabled VB and jumps to the bootloader's entry point. This process initiates the usual sequence of chain loading until the OS is finally loaded into a VB. The OS reads the parameters of \sys, namely, the number of bits of virtual address, the number and sizes of the virtual block size classes, and the maximum number of memory clients supported by the system, to initialize its memory management subsystem.

\noindent
\textbf{Process Creation. }When a binary is executed, the OS creates a new process by associating it with one of the available client IDs. For each segment in the binary (e.g., code, static data), the OS 1)~enables the smallest VB that can fit the contents of the segment and associates the VB with the appropriate properties using the \enablevb instruction, 2)~attaches itself to the VB with write permissions using the \attachvb instruction, 3)~copies the contents from the application binary into the VB, and 4)~detaches itself from the VB using the \detachvb instruction. The OS then attaches the client to the newly enabled VBs and jumps to program's entry point.

\noindent
\textbf{Shared Libraries. }
The OS loads the executable code of each shared library into a separate VB.  Each process needs to attach to a private VB to store shared library data. In order to enable position independent shared library code, one possible solution for \sys  is to satisfy two conditions. First, \sys makes sure that the shared VB of the library code and the private VB that contains any per-process data that the shared library requires are placed in two consecutive entries in the \cvt of the process (e.g., shared code VB at \cvt[N] and private data VB at \cvt[N+1]). Second, \sys links the library code such that the addresses of data references use [\cvt index+1] so that they point to the CVT index of the private data VB in each process. To enable this, VBI needs the ISA to support a \cvt-relative addressing mode, similar to PC-relative addressing in current systems. This solution avoids considerable load-time relocation for each data reference, although VBI can use relocations in the same manner as current systems. After process creation, the OS iterates over the list of shared libraries requested by the process. For each shared library, the OS attaches the client to the corresponding library code and data VBs following the conditions mentioned above.


\noindent
\textbf{Process Destruction. }
When a process terminates, for each VB attached to the process, the OS 1)~detaches the client from the VB (using \detachvb) and 2)~disables the VB if no other process is attached to the VB (using \disablevb). After completing these steps, the OS frees the client ID for reuse.

\noindent
\textbf{Process Forking. }
When a process forks, all of its memory state must be replicated for the newly created process. In \sys, forking entails creating copies of all the VBs attached to a process. To reduce the overhead of this operation, \sys introduces the following instruction:
\begin{center}
\vspace{-5pt}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{tabular}{rl}
\toprule
\clonevb & \tt SVBID, DVBID\\
\bottomrule
\end{tabular}
\vspace{-5pt}
\end{center}
\clonevb \sgdel{essentially} instructs \sys to make the destination VB \texttt{DVBID} a clone of the source VB \texttt{SVBID}. When forking a process, the CVT entries of the parent process are copied into the CVT of the child process so that all VBs have the same CVT index in both processes. This maintains the validity of the pointers in the child VBs after cloning. To efficiently implement \clonevb, the MTL marks all the translation structures and the physical pages of the VBs as copy-on-write and lazily copies the relevant regions if they receive a write operation. In our current implementation of CoW, the CVT index of the VB in both processes needs to be the same to keep CVT-based references in the shared VBs valid. In the case of memory deduplication where the VBs do not have the same CVT index, CoW can not be performed under VBI. However, CoW can still be applied in scenarios such as process forking where the child process VBs are copied at the same CVT index as the parent process.


\subsection{\mtlfull}
\label{sec:mtl}


\subsubsection{\vit (\vitshort)}
\label{sec:vit}

For each VB, the VIT stores 1)~the \emph{enable} bit that indicates if the VB is currently enabled, 2)~a bit vector of VB properties, 3)~the type of translation structure used to map the VB to physical memory, and 4)~a pointer to the translation structure. For ease of access, the MTL maintains a separate VIT for each size class. The unique ID of a VB within its size class is used as an index into the corresponding VIT. 
When a VB is enabled (using \textcolor{blue}{\enablevb}), the MTL sets the \emph{enabled} bit of the entry corresponding to the VB in the VIT of the corresponding size class and updates the \texttt{props} of the VB. The type and pointer of the translation structure are updated at the time of physical memory allocation (\secref{sec:flexible-translations}).


\sys limits the size of each \vit by storing entries only up to the entry of the enabled VB with the largest ID. The OS ensures that the table does not become prohibitively large by reusing previously disabled VBs for subsequent requests. Once a VB is disabled (using \textcolor{blue}{\disablevb}), \sys deallocates VB's translation structures and frees the physical memory allocated to the disabled VB. To avoid stale data in the cache, all of the VB's data is invalidated in the cache \emph{before} reusing the VB. Therefore, no process would be able to access or point to the stale data of a disabled VB. If the system does not need to immediately reuse a given VB (i.e., other free VBs of the same size are available), the cache clean-up can be performed lazily in the background.

%The \textcolor{blue}{\enablevb} instruction 1) adds a new entry to the VIT corresponding to the size class, 2) stores the \texttt{props} of the VB in the newly added entry, and 3) updates the type and pointer to the translation structure of the new VB (explained in Section~\ref{sec:delayed-allocation}). \textcolor{blue}{\disablevb} instruction sets the \emph{enable} bit to zero in VIT entry of the VB. %associated with the VB from the VIT of its size class.


\textbf{Base Address Translation in \sys. }\shepherd{Our base mechanism for VBI-to-physical address translation uses multi-level tables similar to \xeightsix~\cite{pagewalk}}. However, unlike the %512-ary 
4-level page tables in \xeightsix, \sys uses %32-ary 
tables with varying number of levels according to the size of the VB---a 4~KB VB needs zero levels while a 128~KB VB has one level of translation table and so on. The lower number of table levels for smaller VBs reduces the number of required memory accesses to recover from a TLB miss. For each VB, \vitshort stores a pointer to the address of the root of the multi-level table or the physical address of the data for VBs that have zero table levels. As shown in Figure~\ref{fig:vbi-uarch}, \sys performs address translation in parallel with the LLC access. \shepherd{When the \mtl receives the VBI address of a cache line for address translation, it extracts the VB size class, the ID of the VB, and the offset of the cache line inside the VB (Figure~\ref{fig:virtual-address}).} The \mtl then fetches the \vitshort entry of the corresponding VB using the ID and determines the base address of the translation structure for the VB stored in the \vit entry. The \mtl then uses the offset to traverse the translation structure of the VB and determine the physical address of the cache line. \mtl employs a \vitshort cache, translation look-aside buffer (TLB), and a small page-walk cache to speedup these translations.

\textbf{Base Memory Allocation Mechanism. }
The \mtl allocates memory using a buddy algorithm~\cite{knowlton65} customized to the size classes of \sys (which includes 4~KB pages) and performs allocations and mappings at these granularities. Flexible address translation structures chosen for each VB defines the granularity and stores the virtual-to-physical address mapping information in the VB's address translation structure.

\subsubsection{Delayed Physical Memory Allocation}
\label{sec:delayed-allocation}

As described in \secref{sec:optimizations}, \sys delays physical memory allocation for a VB (or a region of VB) until a dirty cache line from that region is evicted from the last-level cache. 
\shepherddelay{There are three possibilities when data for a particular VB is not in the physical memory. 
First, when the process accesses the VB in the physical memory for the first time, it is safe to return a zeroed cache line (without allocating physical memory to the VB). This is because even if physical memory were allocated immediately on the first access to the VB, a read right after allocation would still not return meaningful data. Second, when the process accesses a VB that has been allocated (i.e., mapped) before but has been swapped out of memory, \sys uses a system call to ask the OS to read the necessary pages from storage and allocate them in the memory before the access is performed. Third, when the process accesses file-mapped memory, \sys maps each file-mapped memory region to a VB and marks the VB as file-mapped. Upon a page fault to a file-mapped VB, the MTL uses a system call to read and allocate the necessary pages into the physical memory prior to performing the memory access. Therefore, delayed physical memory allocation does not apply to file-mapped or swapped-out VBs.}

To implement the delayed physical memory allocation mechanism in \sys, upon enabling a new VB, \sys does not immediately allocate physical memory to the VB. On an LLC miss, \sys checks the corresponding VIT entry to determine if physical memory has been allocated. If not, \sys simply returns a zero cache line to the processor. 

\shepherddelay{On a dirty cache line eviction, if physical memory is not yet allocated for the VB, \sys allocates physical memory first and then performs the writeback. If enough physical memory is available, \sys tries to allocate the entire VB as a single direct segment using the smallest size class that fits the VB, in order to reduce address translation overhead. If not enough contiguous physical memory is available for the entire VB, VBI allocates the VB at the granularity of equally-sized regions, where the region size is determined by the largest size class that can be allocated contiguously in physical memory.  Note that VBI allocates only the region of the VB containing the evicted cache line, and that another region is allocated only when the first writeback to that region occurs.} Since writebacks are not on the critical path of the execution, this approach results in minor performance overhead (as shown in our evaluations in Section~\secref{sec:4k-perf}).


\subsubsection{Flexible Translation Structure Types}
\label{sec:flexible-translations}
\sys chooses from three types of address translation structures for each VB depending on the needs of the VB and the availability of the physical memory. The first type \emph{directly} maps the VB to physical memory when enough contiguous memory is available. With this mapping, a single TLB entry is sufficient to maintain the translation for the entire VB. The second type of mapping uses a single-level table where the VB is divided into equal-sized blocks of one of the supported size classes. Each entry in the table maintains the mapping for the corresponding block. This mapping exploits the fact that majority of the data structures are densely allocated inside their respective VBs. With single-level tables, the mapping for any region of the VB can be retrieved with a single memory access. The third type of mapping suitable for sparsely allocated VBs is similar to the \emph{multi-level table} approach employed by Intel architectures but with varying number of levels (as discribed in \secref{sec:mtl}).

The implementation of flexible address translation structures in our evaluations statically chooses a translation structure type based on the size of the VB. Each 4~KB VB is directly mapped. 128~KB and 4~MB VBs use a single-level table. VBs of higher size use multi-level table with as many levels as necessary to map the VB using 4~KB pages. The \emph{early reservation} optimizations explained in next section improve upon this static policy by using blocks of different sizes chosen from the set of supported size classes. While our evaluations assume page-table-like translation structures of varying depth, VBI supports other schemes that prior works demonstrate the benefits of (e.g., customized data structures for specific applications~\cite{vm19}).

Similar to \xeightsix, \sys uses multiple types of TLBs to cache mappings of different granularity. However, the type of translation structure used for a VB is stored in the \vitshort and is cached in the on-chip \vitshort Cache. This information enables \sys to access the right type of TLB. For a fair comparison, our evaluations use the same TLB type and size for all baselines and variants of \sys.

\subsubsection{Early Reservation of Physical Memory}
\label{sec:early-reservation}

This optimization is inspired by prior work on super-page management~\cite{reserve} 
to reserve a larger contiguous region of memory than the requested size and upgrade the allocated pages to larger super pages when enough contiguous pages are allocated in that region. We extend this idea to reserve physical memory for the entire VB at the time of physical memory allocation and consider the VB as directly mapped by serving the future memory allocation requests for that VB in the contiguous reserved region. To implement this approach in \sys, at the time of the first physical memory allocation request for a VB, the \mtl checks if there is enough contiguous free space that can fit the entire VB. If so, it allocates the requested memory from that region and marks any free blocks in that region as reserved for that specific VB. When allocating physical memory for a VB, the \mtl prioritizes free blocks in the following order: 1)~free blocks reserved for the VB that is demanding allocation, 2)~unreserved free blocks, and 3)~free blocks reserved for other VBs.
A VB is then considered directly mapped as long as all its allocated memory is mapped to a single contiguous region of memory, thereby requiring just a single TLB entry for the entire VB. To support this mechanism, \sys uses the Buddy algorithm~\cite{buddy,knowlton65} to manage free and reserved pages of different power-of-2 sizes. If there is not enough contiguous physical memory available to fit the entire VB, the early reservation mechanism allocates the VB sparsely by reserving blocks of the largest size class that can be allocated contiguously. This enables \sys to benefit from larger mapping granularities (from the set of supported size classes~\secref{sec:vb-detail}) and therefore minimize the address translation latency.

\subsubsection{Hardware Implementation}

We envision the MTL as software running on a programmable low-power core within the memory controller. While conventional OSes are responsible for memory allocation, virtual-to-physical mapping and ensuring protection, the MTL does not need to deal with protection, so we expect the MTL code to be simpler than typical OS memory management software. The complexity of the MTL hardware is similar to that of prior proposals like Pinnacle~\cite{pinnacle} (commercially available) and Page Overlays~\cite{page_overlays}, which perform memory allocation and remapping in the memory controller. While both Pinnacle and Page Overlays are hardware solutions, VBI provides flexibility by making the MTL programmable, thereby allowing software updates for different memory management policies (e.g., address translation, mapping, migration, scheduling, garbage collection, etc). Our goal in this work is to understand the potential of hardware-based memory allocation and virtual to physical address translation. We plan to build a working MTL prototype with full system stack support in future work.

\subsection{Upgrade and Downgrade of VB Size Class }
\label{sec:resize}

The size of a VB can grow or shrink in \sys. When a VB grows, \sys: 1) enables a larger VB with a sparse translation structure, 2) copies the virtual-to-physical mapping information of the old VB into the new VB’s translation structure so that, for the old data, it points to the right place in physical memory, and 3) maps the new regions of the VB to the physical memory sparsely and the mapping information for the new regions are added to the translation structure of the VB. The old VB and its associated states are deallocated. In \sys, VBs do not need to be contiguously allocated in physical memory and can grow sparsely. \sys will keep the sparsely allocated regions mapped to the same VB ID. To shrink a VB, the \mtl enables a new smaller VB and copies the mapping information of the occupied regions of the VB to the translation structure of the new VB.



\subsection{Flexibility to Support New Workloads}
\label{sec:flexibility}

VBI chooses the smallest available VB size that fits the needs of each memory allocation. If the available VB size classes are larger than the requirements of newly introduced workloads, internal fragmentation may result. VBI avoids fragmentation in physical memory in two ways. First, VBI can use a sparse translation structure to map the VB to physical memory so that the unused regions of the VB can be paged out if required. Second, the early reservation mechanism helps utilizing the unused regions of a VB to allocate other VBs if needed~(\secref{sec:early-reservation}). If a process needs larger VBs than supported, the allocation can be split among smaller VBs with the same permissions and properties. The MTL and the CVT can perform this multiple VB allocation transparently from the process's perspective by maintaining appropriate pointers in the CVT and VIT tables so that the process operates with just one CVT index to access all the VBs.

\subsection{Supporting Virtual Machines}
\label{sec:virtual-machines}

\sys can implement address space isolation between VMs \shepherd{by \emph{partitioning} the global VBI address space among multiple virtual machines and the host OS.} To this end, \sys reserves several bits in the VBI address for the virtual machine ID. Figure~\ref{fig:vaddr-vm} shows how \sys implements this for a system supporting 31 virtual machines (ID 0 is reserved for the host). In the virtual address, the 5 bits following the size class bits are used to denote the virtual machine ID. For every new virtual machine in the system, the host OS assigns a non-zero VM ID to be used by the guest OS while assigning virtual blocks to processes inside the virtual machine. \sys partitions client IDs using a similar approach. With address-space division between VMs, a guest VM is unaware that it is \minp{virtualized}, and it can allocate/deallocate/access VBs without coordinating with host OS. Our model allows for memory sharing where the host OS uses a designated VM ID reserved to mark the set of VBs that can be shared between different VMs or the host OS. However, such sharing requires explicit coordination with host OS.

\begin{figure}[h]
  \centering
  \vspace{-10pt}
  \input{figures/vaddr-vm}
  \caption{Partitioning the virtual address space among multiple virtual machines. The figure uses the 4~GB size class (\texttt{100}) as example.}
  \label{fig:vaddr-vm}
  \vspace{-10pt}
\end{figure}

\subsection{Supporting Multi-Node Systems}
\label{sec:multi-node}

While there are many ways to implement \sys in multi-node systems, our initial approach partitions the available VBs between multiple MTLs (i.e., the memory controllers) in the system such that the higher order bits of the VB ID indicate the home \mtl of the VB. Each MTL manages the physical memory allocation and VBI-to-physical address translation for the set of VBs that map to its physical memory space. Processes have access to the entire physical address space and can allocate memory in any region of memory regardless of which MTL manages the region. Both the properties associated with a VB allocation request and the availability of free physical memory at each \mtl are considered when choosing an appropriate home \mtl for the VB that can satisfy the VB's specified requirements. While the OS can explicitly migrate data between processors by copying data between VBs, the multiple MTLs can also coordinate to efficiently migrate data between processors. SMP--CMP architectures follow the same rules except that there is no distinction between the different MTLs.

==> 8_other_usecases.tex <==
\subsection{Other Applications of VBI}
\label{sec:other-apps}

%\todo{will leave this section in if we have space}

The \sys framework has many broader benefits and applications. We briefly discuss three such applications, where \sys provides a more efficient platform for implementing previously-proposed as well as new mechanisms.

%\subsection{eXpressive Memory.}

\noindent
\textbf{eXpressive Memory. }eXpressive Memory (XMem)~\cite{xmem} is a recently-proposed hardware-software interface that allows applications to pass down data-structure-level semantic information to hardware for improved resource management. \sys allows for the easy implementation of XMem, by allowing an application to request a different VB for each data structure, and by using per-VB properties to manage hardware resources. 

%\subsubsection{LegoOS.}
\noindent
\textbf{LegoOS. }LegoOS~\cite{legoOS} is a new OS architecture that separates the management of disaggregated system resources, namely, processors, memory and storage. The solution argues that such separation allows better consolidation of resources and lower failure rates in data centers. %As mentioned in that paper, 
However, the biggest challenge in realizing LegoOS is the separation of compute and memory monitors, as most modern processors and OSes assume tight integration of compute and memory. \sys enables a clear separation of physical memory management and enables an efficient implementation of the memory monitor as part of LegoOS.

\noindent
\textbf{Cache-only Data Structures}
Given the growing size of on-chip caches, many applications aim
to retain certain critical data structures in the on-chip
caches. However, the techniques available today trying to achieve this
such as page coloring~\cite{} \todo{cite!} and cache partitioning~\cite{intel-cmat}\todo{add reference}
are optimizations on top of and limited to the current framework and do not guarantee cache-only residence.
\sys offers a entirely new optimization opportunity that we call Cache-only Data Structures. If an application marks a VB as
cache-only, the \mtl does not allocate any physical memory for the
VB and avoids evicting cache lines of the VB from the on-chip
cache as much as possible. However, \sys \emph{informs} the
application of cache misses or evictions for the VB through a
software trap and uses a software handler to manage these
events. This approach allows applications to manage on-chip
caches using an approach similar to memcached.

%\subsubsection{Memory Security.}
%
%\sys potentially enables better implementation of mechanisms that aim to protect data of applications and the OS from each other. Intel's SGX~\cite{sgx} can prevent the OS from having direct access to an application's data. However, by controlling the virtual to physical page mapping, the OS can extract side-channel information from page faults in the SGX memory. \sys closes this side channel by taking this control away from the OS, allowing for a more secure and simpler implementation for SGX. In the other direction,  \sys can be used to mitigate Meltdown~\cite{meltdown}, a recently-discovered vulnerability. \sys does not let an application even generate an address of a VB that it is not attached to. As a result, a malicious application can no longer use Meltdown-style attacks to access kernel memory, thereby eliminating the vulnerability in a cleaner and less costly way than Kernel Page Table Isolation~\cite{meltdown}.



==> VBI_ISCA2020/figures/vaddr-gen.tex <==
\begin{tikzpicture}[inner sep=1pt,outer sep=0pt,>=stealth']

\draw [rounded corners=2pt] (0,0) rectangle (8,0.5);
\draw (4,0) -- ++(0,0.5);
\draw (0.8,0) -- ++(0,0.5);

\node at (0.4,0.25) {\small\texttt{100}};
\node at (2.4,0.25) {\small\texttt{VB ID}};
\node at (6,0.25) {\small\texttt{offset}};

\node (s) at (0.4,-0.3) {\small{3b}};
\node (v) at (2.4,-0.3) {\small{29 bits}};
\node (o) at (6,-0.3) {\small{32 bits}};

\draw [->] (s.west) -- (0,-0.3);
\draw [->] (s.east) -- (0.8,-0.3);
\draw [->] (v.west) -- (0.8,-0.3);
\draw [->] (v.east) -- (4,-0.3);
\draw [->] (o.west) -- (4,-0.3);
\draw [->] (o.east) -- (8,-0.3);

\end{tikzpicture}

==> VBI_ISCA2020/figures/vaddr-vm.tex <==
\begin{tikzpicture}[inner sep=1pt,outer sep=0pt,>=stealth', font=\sffamily]

\draw [rounded corners=2pt] (0,0) rectangle (8,0.5);
\draw (4.4,0) -- ++(0,0.5);
\draw (0.8,0) -- ++(0,0.5);
\draw (1.8,0) -- ++(0,0.5);

\node at (0.4,0.25) {\small\texttt{100}};
\node at (1.3,0.25) {\small{\texttt{VM ID}}};
\node at (3.1,0.25) {\small\texttt{VBID}};
\node at (6.2,0.25) {\small\texttt{offset}};

\node (s) at (0.4,-0.3) {\small{3b}};
\node (m) at (1.3,-0.3) {\small{5b}};
\node (v) at (3.1,-0.3) {\small{24 bits}};
\node (o) at (6.2,-0.3) {\small{32 bits}};

\draw [->] (s.west) -- (0,-0.3);
\draw [->] (s.east) -- (0.8,-0.3);
\draw [->] (m.west) -- (0.8,-0.3);
\draw [->] (m.east) -- (1.8,-0.3);
\draw [->] (v.west) -- (1.8,-0.3);
\draw [->] (v.east) -- (4.4,-0.3);
\draw [->] (o.west) -- (4.4,-0.3);
\draw [->] (o.east) -- (8,-0.3);

\end{tikzpicture}

==> VBI_ISCA2020/figures/vbi-addr-gen.tex <==
\begin{tikzpicture}[inner sep=1pt,outer sep=0pt,>=stealth']

\draw [rounded corners=2pt] (0,0) rectangle (8,0.7);
\draw (4.4,0) -- ++(0,0.7);
\draw[dotted] (1.4,0) -- ++(0,0.7);

\node at (2.2, 0.5) {\small\texttt{VBUID}};
\node at (0.7, 0.2) {\footnotesize\color{Gray}\texttt{\emph{SizeID}}};
\node at (2.8, 0.2) {\footnotesize\color{Gray}\texttt{\emph{VBID}}};
\node at (6.2, 0.35) {\small\texttt{offset}};

\draw[->] (1.75, 0.5) -- ++ (-1.7,0);
\draw[->] (2.65, 0.5) -- ++ (1.7,0);

\end{tikzpicture}


==> VBI_ISCA2020/figures/vbi-overview-new.tex <==
\begin{tikzpicture}[>=stealth',font=\small\sffamily]

  \tikzset{block/.style={draw,rounded corners=3pt,minimum height=0.6cm,align=center}};
  \tikzset{acllabel/.style={fill=CornflowerBlue!20,text=RoyalBlue,font=\footnotesize\sffamily}};
  \tikzset{acl/.style={->,rounded corners=2pt}};
  \tikzset{mmap/.style={->,rounded corners=2pt}};
  \tikzset{vb/.style={draw,rounded corners=3pt,minimum height=1.2cm,minimum width=1.3cm,align=center,fill=BrickRed!15}};
  \tikzset{client/.style={draw,rounded corners=3pt,minimum height=1cm,align=center,fill=black!20}};
  
  \node (mml) [block, minimum width=10cm,minimum height=0.8cm,RoyalPurple, fill=RoyalPurple!15] {\normalsize\textbf{Memory Translation Layer}\\\emph{manages physical memory allocation and VBI-to-physical address mapping\vspace{-2pt}}};
  
  \node (pmem1) [block, minimum width=10cm,minimum height=0.6cm, fill=green!10, yshift=-4mm] at (mml.south) {\normalsize\textbf{Physical Memory}};
  %\node (pmem2) [block, minimum width=2.25cm,anchor=west,xshift=0.25cm] at (pmem1.east) {Low Latency\\Memory};
  %\node (pmem3) [block, minimum width=2.75cm,anchor=west,xshift=0.25cm] at (pmem2.east) {High Bandwidth\\Memory};



  \node (vb1) at (mml.north west) [anchor=south west,yshift=5mm,vb] {\textbf{VB 1}\\[-0.5ex]\textbf{\footnotesize{128KB}}\\[1ex]\\[1ex]code\\[-1.5ex]\\\emph{kernel}};
  \node (vb2) at (vb1.east) [anchor=west,xshift=2mm,vb] {\textbf{VB 2}\\[-0.5ex]\textbf{\footnotesize{128KB}}\\[1ex]\\[1ex]data\\[-1.5ex]\\\emph{kernel}};
  \node (vb4) at (vb2.east) [anchor=west,xshift=2mm,minimum width=1.75cm,vb] {\textbf{VB 3}\\[-0.5ex]\textbf{\footnotesize{128KB}}\\[1ex]\emph{Lat-Sen}\\[1ex]data\\[-1.5ex]\\\emph{user}};
  \node (vb5) at (vb4.east) [anchor=west,xshift=2mm,vb] {\textbf{VB 4}\\[-0.5ex]\textbf{\footnotesize{128KB}}\\[0.9ex]\\shared\\[-0.8ex]library\\[0.4ex]\emph{user}};
  \node (vb6) at (vb5.east) [anchor=west,xshift=2mm,vb] {\textbf{VB 5}\\[-0.5ex]\textbf{\footnotesize{128KB}}\\[1ex]\\[1ex]code\\[-1.5ex]\\\emph{user}};
  \node (vb7) at (vb6.east) [anchor=west,xshift=2mm,vb,minimum width=2.4cm] {\textbf{VB 6}\\[-0.5ex]\textbf{\footnotesize{4GB}}\\[1ex]\emph{Band-Sen}\\[1ex]data\\[-1.5ex]\\\emph{user}};
  
       \node at (vb5.south) [yshift=-2mm, xshift=-3mm,text=BrickRed]{\textbf{VBI Address Space}};
  
  \node (hostos) at (vb1.north west) [anchor=south west,minimum width=4cm,yshift=10mm,block] {\textbf{Host Operating System}};
  \node (p1) at (hostos.east) [anchor=west,xshift=15mm,block] {\textbf{Program 2} (native)};

  \node (vl) at (hostos.north west) [anchor=south west,yshift=2mm,minimum width=10cm,align=center] {};
  \node (vllabel) at (vl.west) [anchor=west,xshift=15mm,black!50] {\emph{Virtualization Layer}};
  \draw [dashed,black!50] (vllabel.west) -- (vl.west);
  \draw [dashed,black!50] (vllabel.east) -- (vl.east);

  \node (guestos) at (vl.north west) [anchor=south west,yshift=2mm,minimum width=4cm,block] {\textbf{Guest Operating System}};
  \node (p2) at (guestos.east) [anchor=west,xshift=5mm,block] {\textbf{Program 1} (virtual)};
  
  \draw [rounded corners=5pt,color=CornflowerBlue!30,fill=CornflowerBlue!20] ([yshift=2mm,xshift=-1.5mm]vb1.north west) rectangle ([yshift=8mm,xshift=1.5mm]vb7.north east);

     \fill [BrickRed,fill opacity=0.15,rounded corners=2pt] ([yshift=1mm,xshift=-1.5mm]vb1.north west) rectangle ([yshift=-4mm,xshift=1.5mm]vb7.south east);
     
  

  \draw [acl] ([xshift=-10mm]hostos.south) -- ([xshift=2mm]vb1.north);
  \draw [acl] ([xshift=-3mm]hostos.south) -- ([xshift=0mm]vb2.north);
  \draw [acl] (guestos.west) -- ++(-2mm,0) -- ++(0,-1.7cm) -| ([xshift=-2mm]vb1.north);

  \draw [acl] (p1.south) -- (vb7.north);
  \draw [acl] ([xshift=-2mm]p1.south) -- (vb6.north);
  \draw [acl] ([xshift=-5mm]p1.south) -- ([xshift=1mm]vb5.north);

  \draw [acl] ([xshift=-10mm]p2.south) -- ([xshift=2mm]vb4.north);
  \draw [acl] ([xshift=-7mm]p2.south) -- ([xshift=-1mm]vb5.north);

  %\draw [mmap] (vb1.south) -- (vb1.south|-pmem1.north);
  %\draw [mmap] (vb2.south) -- ([xshift=-5mm]pmem1.north);
  %\draw [mmap] (vb5.south) -- ([xshift=-0mm]pmem1.north);
  %\draw [mmap] (vb6.south) -- ([xshift=10mm]pmem1.north);

  %\draw [mmap,blue] (vb4.south) -- (pmem2.north);
  %\draw [mmap,blue] (vb7.south) -- (pmem3.north);


  \node (l1) [acllabel] at ([yshift=5mm,xshift=-2mm]vb1.north) {X};
  \node (l2) [acllabel,anchor=west] at ([xshift=0.7mm]l1.east) {X};
  \node (l2) [acllabel,anchor=west] at ([xshift=9mm]l1.east) {RW};
  \node (l3) [acllabel,anchor=west] at ([xshift=31mm]l1.east) {RW};
  \node (l4) [acllabel,anchor=west] at ([xshift=42mm]l1.east) {X};
  \node (l4) [acllabel,anchor=west] at ([xshift=48.5mm]l1.east) {X};
  \node (l4) [acllabel,anchor=west] at ([xshift=57.5mm]l1.east) {X};
  \node (l4) [acllabel,anchor=west] at ([xshift=68mm]l1.east) {R};
  
    \node (label) at (l1.east) [yshift=1mm,xshift=86mm,text=RoyalBlue,align=center]{\textbf{\emph{Access}}};
    \node at (label.south) [text=RoyalBlue,align=center]{\textbf{\emph{Permissions}}};

  
\end{tikzpicture}

%%damn it! Finally!

==> VBI_ISCA2020/figures/vbi-uarch.tex <==
\begin{tikzpicture}[>=stealth']\footnotesize

  \tikzset{rounded/.style={draw,rounded corners=2pt}};
  \tikzset{mmlstruct/.style={rounded,align=center,minimum height=1.25cm,inner xsep=5pt}};

  
  \node (app) [rounded,align=left,anchor=south west,font=\tt\footnotesize,yshift=5mm] {
    ...\\
    index = request\_vb(size, props);\\
    x = malloc(index, size);\\
    ...\\
    y = (*x); // \underline{ld reg, index, offset}\\
    ...
  };
  \node at (app.north) [anchor=south] {Application};

  \node (os) at (app.east) [rounded,align=left,anchor=west,font=\tt\footnotesize,xshift=7mm] {
    ...\\
    // identify appropriate VB~~\\
    enable\_vb vid, props\\
    attach vid, cid, RW\\
    // return index to process\\
    ...
  };
  \node at (os.north) [anchor=south] {Operating System};
  

  \node (cpu) at (app.south west) [rounded,anchor=north west,yshift=-8mm,minimum height=1.5cm,minimum width=1.5cm] {CPU};

  \node (cvtcache) at (cpu.east) [rounded,anchor=west,xshift=1cm,minimum height=1.5cm,minimum width=3.5cm] {};
  \node at (cvtcache.north) [anchor=south] {CVT Cache};
  \node (cvtfields) at (cvtcache.north) [anchor=north,font=\scriptsize\tt,minimum width=3.5cm] {Index~~Size~~~VID~~RWX};
  \draw (cvtfields.south west) -- (cvtfields.south east);

  \node (va) at (cpu.south west) [rounded,anchor=north west,yshift=-5mm,minimum height=6mm] {~Size~~~VID~~~~Offset~~};
  \node at (va.south) [anchor=north] {Virtual Address (VA)};

  \node (l1) at (cvtcache.south east) [rounded,anchor=north east,yshift=-5mm,minimum height=6mm,minimum width=2.5cm,align=center] {L1 Cache};

  \node (llc) at (os.east|-cvtcache.north) [rounded,anchor=north east,minimum height=0.7cm,minimum width=3.3cm] {LLC};

  \node (vitcache) at (llc.west|-l1.south) [rounded,anchor=south west,minimum height=1.3cm,minimum width=3.3cm] {};
  \node at (vitcache.south) [anchor=north] {VIT Cache};
  \node (vitfields) at (vitcache.north) [anchor=north,font=\scriptsize\tt,minimum width=3.3cm] {Size~~VID~~Props~Trans};
  \draw (vitfields.south west) -- (vitfields.south east);

  \node (tlb) at (vitcache.south east) [rounded,anchor=south west,xshift=8mm,minimum height=1.3cm,minimum width=1.5cm] {TLBs};

  \node (pw) at (tlb.north) [rounded,anchor=south,yshift=7mm,minimum height=1.3cm,minimum width=1.5cm,align=center] {Trans.\\Walker};

  \node (mc) at (os.north east) [rounded,anchor=north west,xshift=8mm,minimum width=1.5cm,minimum height=1.3cm,align=center] {Memory\\Ctrl.};

  \node (pmem) at (tlb.south east) [rounded,anchor=south west,xshift=8mm,minimum width=1.5cm,minimum height=5.3cm] {};
  \node at (pmem.south) [anchor=north] {Main Memory};

  \node (vlabel) at (pmem) [yshift=2.4cm,minimum width=1.5cm] {VITs};
  \node (clabel) at (pmem) [yshift=1.8cm,minimum width=1.5cm] {CVTs};
  \node (tlabel) at (pmem) [yshift=1cm,align=center,minimum width=1.5cm] {Trans.\\Tables};
  \node (dlabel) at (pmem) [yshift=-1cm,minimum width=1.5cm] {Data};

  \draw ([yshift=-1mm]clabel.south west) -- ([yshift=-1mm]clabel.south east);
  \draw ([yshift=-1mm]vlabel.south west) -- ([yshift=-1mm]vlabel.south east);
  \draw ([yshift=-1mm]tlabel.south west) -- ([yshift=-1mm]tlabel.south east);

  % data path
  \draw [->,rounded] ([yshift=3.5mm]app.south) -- ++(0,-9mm) -| (cpu.north);
  \draw [->,rounded] ([yshift=5.5mm,xshift=-1.5mm]app.east) -- ++(5mm,0) |- (os.west);
  \draw [->,rounded,red] ([yshift=2mm,xshift=-9.5mm]os.east) -- ++(14mm,0) |- (mc.west|-vlabel.west) (mc.east|-vlabel.west) -- ([xshift=2mm]vlabel.west);

  \draw [->,rounded,red,densely dashed] ([yshift=-1mm,xshift=-12mm]os.east) --  ([yshift=-1mm]os.east-|mc.west)  ([yshift=1mm]mc.east) -- ++(6mm,0) |- ([xshift=2mm]clabel.west);%([yshift=-1mm,xshift=2mm]os.east-|clabel.west);
  
  \draw [->] (cpu.south) -- (cpu.south|-va.north) node [midway,left] {\tt\footnotesize offset};
  \draw [->] ([yshift=3mm]cpu.east) -- ([yshift=3mm]cvtcache.west) node [midway,above] {\tt\footnotesize index};
  \draw [->,rounded] ([yshift=-2mm]cvtcache.west) -| ([xshift=5mm]va.north) node [anchor=south west] {\tt\footnotesize size,VID};
  \draw [->,violet] (va.east) -- (l1.west) node [midway,below] {\tt VA};
  \draw [->,violet] (l1.east) -- (l1.east-|vitcache.west);
  \draw [->,rounded,violet] ($(l1.east)!0.5!(l1.east-|vitcache.west)$) |- (llc.west);
  \draw [->,violet] (llc.south) -- (vitcache.north);
  \draw [->,violet] (vitcache.east) -- (tlb.west);
  \draw [->,violet] (tlb.north) -- (pw.south);
  \draw [->,densely dashed] ([xshift=2mm]pw.north) -- ([xshift=2mm]mc.south);
  \draw [->,rounded,blue] ([xshift=4mm]tlb.north west) -- ++(0,4mm) -| ([yshift=3mm,xshift=-3mm]pw.north west) -| ([xshift=-2mm]mc.south) node [anchor=north east] {\tt\footnotesize PA};

  \draw [->,densely dashed,rounded] ([yshift=-2mm]mc.east) -- ++(4mm,0) |- ([xshift=2mm]tlabel.west);
  \draw [->,blue,rounded] ([yshift=-4mm]mc.east) -- ++(2mm,0) |- ([xshift=2mm]dlabel.west);

  \node at (l1.east) [anchor=north west] {miss};
  \node at (llc.south) [anchor=north west] {miss};
  \node at (tlb.north) [anchor=south west] {miss};
  
  \draw [densely dotted,rounded] ([xshift=-8mm,yshift=-2mm]app.south west) -| ([xshift=2mm,yshift=2mm]os.north east);
  \node at ([xshift=-8mm,yshift=-2mm]app.south west) [anchor=south west] {S/W};  
  \node at ([xshift=-8mm,yshift=-2mm]app.south west) [anchor=north west] {H/W};

  \node at ([yshift=-1mm,xshift=4mm]app.south)
        [anchor=south,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 1};

  \node at ([yshift=1mm,xshift=1mm]cpu.east)
        [anchor=west,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 2};

  \node at ([yshift=1mm,xshift=0mm]va.north)
        [anchor=south,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 3};

  \node at ([yshift=1mm,xshift=-1mm]l1.west)
        [anchor=south east,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 4};

  \node at ([yshift=1mm,xshift=-1mm]vitcache.north)
        [anchor=south east,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 5};



  %\node at ([xshift=8mm]cpu.north east) [anchor=east,circle,white,fill=black,inner sep=.5pt] {\footnotesize 2};
  %\node at ([xshift=4mm,yshift=4mm]app.south east) [anchor=east,circle,white,fill=black,inner sep=.5pt] {\footnotesize 1};
  %\node at ([xshift=5mm,yshift=-4mm]cpu.south) [anchor=south,circle,white,fill=black,inner sep=.5pt] {\footnotesize 3};
  %\node at ([xshift=3mm,yshift=-3mm]va.east) [anchor=north,circle,white,fill=black,inner sep=.5pt] {\footnotesize 4};
  %\node at ([xshift=3mm,yshift=-3mm]l1.east) [anchor=north,circle,white,fill=black,inner sep=.5pt] {\footnotesize 4};
\end{tikzpicture}



==> figures/vaddr-gen.tex <==
\begin{tikzpicture}[inner sep=1pt,outer sep=0pt,>=stealth']

\draw [rounded corners=2pt] (0,0) rectangle (8,0.5);
\draw (4,0) -- ++(0,0.5);
\draw (0.8,0) -- ++(0,0.5);

\node at (0.4,0.25) {\small\texttt{100}};
\node at (2.4,0.25) {\small\texttt{VB ID}};
\node at (6,0.25) {\small\texttt{offset}};

\node (s) at (0.4,-0.3) {\small{3b}};
\node (v) at (2.4,-0.3) {\small{29 bits}};
\node (o) at (6,-0.3) {\small{32 bits}};

\draw [->] (s.west) -- (0,-0.3);
\draw [->] (s.east) -- (0.8,-0.3);
\draw [->] (v.west) -- (0.8,-0.3);
\draw [->] (v.east) -- (4,-0.3);
\draw [->] (o.west) -- (4,-0.3);
\draw [->] (o.east) -- (8,-0.3);

\end{tikzpicture}

==> figures/vbi-uarch.tex <==
\begin{tikzpicture}[>=stealth']\footnotesize

  \tikzset{rounded/.style={draw,rounded corners=2pt}};
  \tikzset{mmlstruct/.style={rounded,align=center,minimum height=1.25cm,inner xsep=5pt}};

  
  \node (app) [rounded,align=left,anchor=south west,font=\tt\footnotesize,yshift=5mm] {
    ...\\
    index = request\_vb(size, props);\\
    x = malloc(index, size);\\
    ...\\
    y = (*x); // \underline{ld reg, index, offset}\\
    ...
  };
  \node at (app.north) [anchor=south] {Application};

  \node (os) at (app.east) [rounded,align=left,anchor=west,font=\tt\footnotesize,xshift=7mm] {
    ...\\
    // identify appropriate VB~~\\
    enable\_vb vid, props\\
    attach vid, cid, RW\\
    // return index to process\\
    ...
  };
  \node at (os.north) [anchor=south] {Operating System};
  

  \node (cpu) at (app.south west) [rounded,anchor=north west,yshift=-8mm,minimum height=1.5cm,minimum width=1.5cm] {CPU};

  \node (cvtcache) at (cpu.east) [rounded,anchor=west,xshift=1cm,minimum height=1.5cm,minimum width=3.5cm] {};
  \node at (cvtcache.north) [anchor=south] {CVT Cache};
  \node (cvtfields) at (cvtcache.north) [anchor=north,font=\scriptsize\tt,minimum width=3.5cm] {Index~~Size~~~VID~~RWX};
  \draw (cvtfields.south west) -- (cvtfields.south east);

  \node (va) at (cpu.south west) [rounded,anchor=north west,yshift=-5mm,minimum height=6mm] {~Size~~~VID~~~~Offset~~};
  \node at (va.south) [anchor=north] {Virtual Address (VA)};

  \node (l1) at (cvtcache.south east) [rounded,anchor=north east,yshift=-5mm,minimum height=6mm,minimum width=2.5cm,align=center] {L1 Cache};

  \node (llc) at (os.east|-cvtcache.north) [rounded,anchor=north east,minimum height=0.7cm,minimum width=3.3cm] {LLC};

  \node (vitcache) at (llc.west|-l1.south) [rounded,anchor=south west,minimum height=1.3cm,minimum width=3.3cm] {};
  \node at (vitcache.south) [anchor=north] {VIT Cache};
  \node (vitfields) at (vitcache.north) [anchor=north,font=\scriptsize\tt,minimum width=3.3cm] {Size~~VID~~Props~Trans};
  \draw (vitfields.south west) -- (vitfields.south east);

  \node (tlb) at (vitcache.south east) [rounded,anchor=south west,xshift=8mm,minimum height=1.3cm,minimum width=1.5cm] {TLBs};

  \node (pw) at (tlb.north) [rounded,anchor=south,yshift=7mm,minimum height=1.3cm,minimum width=1.5cm,align=center] {Trans.\\Walker};

  \node (mc) at (os.north east) [rounded,anchor=north west,xshift=8mm,minimum width=1.5cm,minimum height=1.3cm,align=center] {Memory\\Ctrl.};

  \node (pmem) at (tlb.south east) [rounded,anchor=south west,xshift=8mm,minimum width=1.5cm,minimum height=5.3cm] {};
  \node at (pmem.south) [anchor=north] {Main Memory};

  \node (vlabel) at (pmem) [yshift=2.4cm,minimum width=1.5cm] {VITs};
  \node (clabel) at (pmem) [yshift=1.8cm,minimum width=1.5cm] {CVTs};
  \node (tlabel) at (pmem) [yshift=1cm,align=center,minimum width=1.5cm] {Trans.\\Tables};
  \node (dlabel) at (pmem) [yshift=-1cm,minimum width=1.5cm] {Data};

  \draw ([yshift=-1mm]clabel.south west) -- ([yshift=-1mm]clabel.south east);
  \draw ([yshift=-1mm]vlabel.south west) -- ([yshift=-1mm]vlabel.south east);
  \draw ([yshift=-1mm]tlabel.south west) -- ([yshift=-1mm]tlabel.south east);

  % data path
  \draw [->,rounded] ([yshift=3.5mm]app.south) -- ++(0,-9mm) -| (cpu.north);
  \draw [->,rounded] ([yshift=5.5mm,xshift=-1.5mm]app.east) -- ++(5mm,0) |- (os.west);
  \draw [->,rounded,red] ([yshift=2mm,xshift=-9.5mm]os.east) -- ++(14mm,0) |- (mc.west|-vlabel.west) (mc.east|-vlabel.west) -- ([xshift=2mm]vlabel.west);

  \draw [->,rounded,red,densely dashed] ([yshift=-1mm,xshift=-12mm]os.east) --  ([yshift=-1mm]os.east-|mc.west)  ([yshift=1mm]mc.east) -- ++(6mm,0) |- ([xshift=2mm]clabel.west);%([yshift=-1mm,xshift=2mm]os.east-|clabel.west);
  
  \draw [->] (cpu.south) -- (cpu.south|-va.north) node [midway,left] {\tt\footnotesize offset};
  \draw [->] ([yshift=3mm]cpu.east) -- ([yshift=3mm]cvtcache.west) node [midway,above] {\tt\footnotesize index};
  \draw [->,rounded] ([yshift=-2mm]cvtcache.west) -| ([xshift=5mm]va.north) node [anchor=south west] {\tt\footnotesize size,VID};
  \draw [->,violet] (va.east) -- (l1.west) node [midway,below] {\tt VA};
  \draw [->,violet] (l1.east) -- (l1.east-|vitcache.west);
  \draw [->,rounded,violet] ($(l1.east)!0.5!(l1.east-|vitcache.west)$) |- (llc.west);
  \draw [->,violet] (llc.south) -- (vitcache.north);
  \draw [->,violet] (vitcache.east) -- (tlb.west);
  \draw [->,violet] (tlb.north) -- (pw.south);
  \draw [->,densely dashed] ([xshift=2mm]pw.north) -- ([xshift=2mm]mc.south);
  \draw [->,rounded,blue] ([xshift=4mm]tlb.north west) -- ++(0,4mm) -| ([yshift=3mm,xshift=-3mm]pw.north west) -| ([xshift=-2mm]mc.south) node [anchor=north east] {\tt\footnotesize PA};

  \draw [->,densely dashed,rounded] ([yshift=-2mm]mc.east) -- ++(4mm,0) |- ([xshift=2mm]tlabel.west);
  \draw [->,blue,rounded] ([yshift=-4mm]mc.east) -- ++(2mm,0) |- ([xshift=2mm]dlabel.west);

  \node at (l1.east) [anchor=north west] {miss};
  \node at (llc.south) [anchor=north west] {miss};
  \node at (tlb.north) [anchor=south west] {miss};
  
  \draw [densely dotted,rounded] ([xshift=-8mm,yshift=-2mm]app.south west) -| ([xshift=2mm,yshift=2mm]os.north east);
  \node at ([xshift=-8mm,yshift=-2mm]app.south west) [anchor=south west] {S/W};  
  \node at ([xshift=-8mm,yshift=-2mm]app.south west) [anchor=north west] {H/W};

  \node at ([yshift=-1mm,xshift=4mm]app.south)
        [anchor=south,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 1};

  \node at ([yshift=1mm,xshift=1mm]cpu.east)
        [anchor=west,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 2};

  \node at ([yshift=1mm,xshift=0mm]va.north)
        [anchor=south,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 3};

  \node at ([yshift=1mm,xshift=-1mm]l1.west)
        [anchor=south east,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 4};

  \node at ([yshift=1mm,xshift=-1mm]vitcache.north)
        [anchor=south east,circle,white,fill=black,inner sep=1pt]
        {\scriptsize 5};



  %\node at ([xshift=8mm]cpu.north east) [anchor=east,circle,white,fill=black,inner sep=.5pt] {\footnotesize 2};
  %\node at ([xshift=4mm,yshift=4mm]app.south east) [anchor=east,circle,white,fill=black,inner sep=.5pt] {\footnotesize 1};
  %\node at ([xshift=5mm,yshift=-4mm]cpu.south) [anchor=south,circle,white,fill=black,inner sep=.5pt] {\footnotesize 3};
  %\node at ([xshift=3mm,yshift=-3mm]va.east) [anchor=north,circle,white,fill=black,inner sep=.5pt] {\footnotesize 4};
  %\node at ([xshift=3mm,yshift=-3mm]l1.east) [anchor=north,circle,white,fill=black,inner sep=.5pt] {\footnotesize 4};
\end{tikzpicture}


